Evaluating LLMs' Mathematical and Coding Competency through Ontology-guided Interventions

Recent advancements in Large Language Models (LLMs) have showcased striking results on existing logical reasoning benchmarks, with some models even surpassing human performance. However, the true depth of their competencies and robustness in reasoning tasks remains an open question. To this end, in this paper, we focus on two popular reasoning tasks: arithmetic reasoning and code generation. Particularly, we introduce (i) a general ontology of perturbations for math and coding questions, (ii) a semi-automatic method to apply these perturbations, and (iii) two datasets, GSMORE and HUMANEVAL-CORE, respectively, of perturbed math and coding problems to probe LLM capabilities in numeric reasoning and coding tasks. Through comprehensive evaluations of both closed-source and open-source LLMs, we show a significant performance drop across all the models against the perturbed questions, suggesting that the current LLMs lack robust problem solving skills and structured reasoning abilities in many areas, as defined by our ontology. We open-source the datasets and source codes at: https://github.com/declare-lab/LLM-ReasoningTest.

==> related-works.tex <==
\section{Related Work}
\paragraph{Instruction Augmentation for Fine-Tuning.}
Our research is inspired by the Evol-Instruct approach by WizardLM~\citep{xu2023wizardlm} and its subsequent extensions. WizardLM's method focused on refining instruction data by increasing its complexity and diversity from seed instruction data. This was achieved by feeding heuristic prompts to existing large language models (LLMs) to generate the data. A notable extension of this work is `WizardMath'~\citep{luo2023wizardmath}, which applies the same methodology to the GSM8K dataset. Similarly, `WizardCoder'~\citep{luo2023wizardcoder} enhanced code-specific data using this approach. However, these studies primarily emphasized increasing diversity and depth in their instruction prompts to ChatGPT, without specifically testing particular abilities. Additionally, the perturbed questions in their approach could change in various ways, lacking the controlled, unidirectional change characteristic of our method. Another critical aspect to consider is that their dataset has not undergone human verification and correction, raising concerns about the reliability and quality of the data.
% Instruction following evaluation: alpaca farm, instruct-bench(as a evaluation paper) 



% Check the citations of beyond accuracy
\paragraph{Robustness and Behavior Testing.}
The field of research has increasingly shifted its focus towards evaluating models on criteria beyond the mere held-out accuracy of datasets. This shift is partly due to concerns about data contamination \citep{golchin2023time} and reliability of the model performance \citep{raj2023measuring}. Inspired by the concept of behavior testing in software engineering, the CheckList \citep{ribeiro2020beyond} methodology was introduced. This approach allows for the rapid generation of diverse, task-agnostic test cases to assess model performance. Building on this trend, several studies have explored using syntactic features to create question perturbations, aiming to test a model's robustness. However, there is a noticeable gap in automatically generating such perturbations for the field of logic reasoning. This gap exists because creating datasets in domains like math and coding is challenging due to their complex data structures. Our work addresses this gap. While maintaining the generality of the perturbation ontology to logic reasoning tasks, we also integrate task-specific features into this ontology, enabling the creation of more nuanced and relevant perturbations.


\paragraph{Counterfactual Question Generation.}
Several research efforts have been directed towards generating counterfactual questions as a means to both enrich datasets and evaluate model performance. For instance, the MetaMath~\citep{yu2023metamath} project has demonstrated various methods to rephrase original questions to different formats, thereby improving the model's ability in complex mathematical reasoning. Similarly, in Reasoning or Reciting~\citep{wu2023reasoning}, authors developed counterfactual datasets specifically designed to test the limitations of large language models (LLMs) in reasoning. They employed fake questions to ascertain if the models could transfer reasoning skills to unfamiliar contexts. In contrast to these approaches, our work diverges significantly. Rather than focusing on creating fake or hypothetical questions, our methodology involves crafting realistic questions that are explicitly designed to assess and challenge the model's knowledge base and reasoning capabilities. This approach aims to provide a more practical and direct assessment of model performance in real-world scenarios.


% taking a step back to move forward
% cider, 
% CLOMO: Counterfactual Logical Modification with Large Language Models
% Universal and Transferable Adversarial Attacks on Aligned Language Models
% REMASK

% Math Dataset:
% GSM8K, MAWPS, AQuA, SVAMP, MathQA
%\input{latex/new-ontology}
% \input{latex/}
% We categorize the various perturbations to different dataset types that necessitate reasoning. Initially, we brainstorm to identify broad categories of perturbations. Subsequently, we integrate these categories into a unified ontology applicable to both coding and mathematical datasets. For each dataset, we devise specific implementations based on these broad intervention categories.


% Useless below
% \subsection{Evaluation on Perturbed Questions}
% \paragraph{Response Generation.}
% To assess the performance of Large Language Models (LLMs), we employ a variety of prompting techniques to generate their responses. Once these responses are generated, we then proceed to evaluate each domain's quality and correctness. 

% \paragraph{Problem Solving Questions.}
%  For math-related problem-solving questions, we manually label the answers. This involves a detailed review of each question and its corresponding answer to ensure accuracy and relevance.

% \paragraph{Instruction Following Questions.}

% The evaluation process for instruction-following questions is twofold. Firstly, we automatically check if the generated question is correct and aligns with the original content. Secondly, we assess whether the response adheres to the specific instructions or requirements outlined in the perturbed question. This assessment is primarily conducted by GPT-4, which evaluates the alignment of the LLM's output with the set instructions.

% \paragraph{Robustness Questions and Non-Standard Answers.}

% For robustness-related questions and other questions that do not have a straightforward or standard answer, we conduct a manual evaluation. This involves a thorough review of each response generated by the LLMs to assess their appropriateness, accuracy, and relevance to the given question. Manual evaluation is crucial here, as these types of questions often require nuanced judgment that automated systems may not fully capture.

% TODO: categorization and test case may not have standard answer
% Potential intervention Types:
% GSM8k: predict mask information, distraction can be arrange the information in temporal sequence.
% Human_eval: generalize input range; write modularized code; write fewer code; write code comment; Self Define rules;


